Training Free Guided Flow Matching with Optimal Control

Controlled generation with pre-trained Diffusion and Flow Matching models has vast applications. One strategy for guiding ODE-based generative models is through optimizing a target loss $R(x_1)$ while staying close to the prior distribution. Along this line, some recent work showed the effectiveness of guiding flow model by differentiating through its ODE sampling process. Despite the superior performance, the theoretical understanding of this line of methods is still preliminary, leaving space for algorithm improvement. Moreover, existing methods predominately focus on Euclidean data manifold, and there is a compelling need for guided flow methods on complex geometries such as SO(3), which prevails in high-stake scientific applications like protein design. We present OC-Flow, a general and theoretically grounded training-free framework for guided flow matching using optimal control. Building upon advances in optimal control theory, we develop effective and practical algorithms for solving optimal control in guided ODE-based generation and provide a systematic theoretical analysis of the convergence guarantee in both Euclidean and SO(3). We show that existing backprop-through-ODE methods can be interpreted as special cases of Euclidean OC-Flow. OC-Flow achieved superior performance in extensive experiments on text-guided image manipulation, conditional molecule generation, and all-atom peptide design.

==> micro.tex <==
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}
\usepackage{url}
\usepackage{verbatim} % allows multiline comments
\usepackage{graphicx}
% \usepackage{caption} 
\usepackage{multirow}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{xspace}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{times}
\usepackage{xr}
\usepackage{bbm}
\usepackage{bm}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{hyperref}       % hyperlinks
\usepackage{multicol}
\usepackage{tabularx}
\usepackage{perpage} %the perpage package
\MakePerPage{footnote} %the perpage package command
\usepackage{wrapfig}
\usepackage{makecell}

% \usepackage[skip=0pt]{caption}

% \usepackage{algorithm}
% \usepackage[noend]{algpseudocode}
% \usepackage{float}




\newcommand{\jiaxuan}[1]{{{\textcolor{blue}{[Jiaxuan: #1]}}}}
\newcommand{\rex}[1]{{{\textcolor{magenta}{[Rex: #1]}}}}
\newcommand{\jure}[1]{{{\textcolor{red}{[Jure: #1]}}}}

\newcommand{\xhdr}[1]{{\noindent\bfseries #1}.}
\newcommand{\todo}[1]{{\textcolor{red}{TODO: #1}}}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\CITE}{{\textcolor{red}{[CITE]}}}

\newcommand{\hide}[1]{}

\newcommand{\nedge}{k}
\newcommand{\mb}{\mathbf}
% \newcommand{\mc}{\mathcal}
\newcommand{\cut}[1]{}
%\newcommand{\xhdr}[1]{\vspace{1.7mm}\noindent{{\bf #1}}}
\newcommand{\casc}{{\mathbf{t}}}
\newcommand{\alphs}{{\mathbf{A}}}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{observation}{\textbf{Observation}}
\newcommand{\xsketch}{\noindent {\it Proof Sketch.}}
\newcommand{\netinf}{{\textsc{Net\-Inf}}\xspace}
\newcommand{\multitree}{{\textsc{Multi\-Tree}}\xspace}
\newcommand{\netrate}{{\textsc{Net\-Rate}}\xspace}
\newcommand{\connie}{{\textsc{Co\-nNIe}}\xspace}
\newcommand{\maxinf}{{\textsc{Max\-Inf}}\xspace}
\newcommand{\expo}{{\textsc{Exp}}\xspace}
\newcommand{\pow}{{\textsc{Pow}}\xspace}
\newcommand{\ray}{{\textsc{Ray}}\xspace}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\versus}{\emph{vs.}\xspace}
\newcommand{\unobs}{{\infty}}
\newcommand\T{\rule{0pt}{2.6ex}}
\newcommand\B{\rule[-1.2ex]{0pt}{0pt}}
% \DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\Bernoulli}{Bernoulli}
\DeclareMathOperator{\Multimonial}{Multimonial}
\DeclareMathOperator{\NodeMerge}{NodeMerge}
\DeclareMathOperator{\NodeSplit}{NodeSplit}
\DeclareMathOperator{\Uniform}{Uniform}
\DeclareMathOperator{\Degree}{Degree}
\DeclareMathOperator{\GCN}{GCN}



\newcommand{\V}{\mathcal{V}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\G}{\mathcal{G}}



\newcommand{\name}{UbiGraph\xspace}

\newcommand{\ba}{Barab\'asi-Albert\xspace}
\newcommand{\er}{Erd\H{o}s-R\'enyi\xspace}
\newcommand{\ws}{Watts-Strogatz\xspace}

==> tabs/qm9_full.tex <==
\begin{table}[ht]
\centering
\caption{Guided generation metrics on QM9.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccccccccc@{}}
\toprule
Property & \multicolumn{4}{c}{$\alpha$ / Bohr³} & \multicolumn{4}{c}{$\Delta\varepsilon$ / meV} & \multicolumn{4}{c}{$\varepsilon_\text{HOMO}$ / meV} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(l){10-13} 
Metric & MAE & ASP & MSP & ValP & MAE & ASP & MSP & ValP & MAE & ASP & MSP & ValP \\ \midrule
Ours ($\gamma=0.01$) & \textbf{1.383} & 94.8 & 64.4 & 86.2 & 367 & 95.2 & 67.9 & 88.2 & \textbf{183} & 95.2 & 65.8 & 86.3 \\
Ours ($\gamma=10$) & 1.557 & \textbf{96.0} & \textbf{69.9} & 88.6 & 365 & \textbf{96.1} & 70.5 & \textbf{89.8} & 188 & \textbf{96.1} & \textbf{69.8} & 87.9 \\
D-Flow & 1.566 & 95.9 & 69.0 & \textbf{88.7} & \textbf{355} & 95.8 & \textbf{70.7} & 88.1 & 205 & 95.7 & \textbf{69.8} & \textbf{88.7} \\
Flowgrad & 2.484 & 95.4 & 65.6 & 83.6 & 517 & 95.5 & 68.3 & 83.1 & 273 & 95.3 & 66.2 & 85.0 \\
EquiFM & 8.969 & 98.6 & 87.2 & 94.7 & 1439 & 98.6 & 87.4 & 94.8 & 622 & 98.6 & 87.4 & 94.8 \\ \midrule

Property & \multicolumn{4}{c}{$\varepsilon_\text{LUMO}$ / meV} & \multicolumn{4}{c}{$\mu$ / D} & \multicolumn{4}{c}{$c_v$ / ($\text{cal}\cdot\text{K}^{-1}\cdot\text{mol}^{-1}$)} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(l){10-13} 
Metric & MAE & ASP & MSP & ValP & MAE & ASP & MSP & ValP & MAE & ASP & MSP & ValP \\ \midrule
Ours ($\gamma=0.01$) & 342 & 95.3 & 68.5 & 87.6 & \textbf{0.314} & 95.8 & 68.0 & 88.4 & \textbf{0.819} & 95.2 & 67.1 & \textbf{89.5} \\
Ours ($\gamma=10$) & \textbf{339} & \textbf{96.1} & \textbf{70.8} & 88.8 & 0.320 & 96.1 & 70.1 & 89.0 & 0.852 & \textbf{96.1} & 68.9 & 88.6 \\
D-Flow & 346 & 95.9 & 70.6 & \textbf{89.3} & 0.330 & \textbf{96.2} & \textbf{71.3} & \textbf{89.2} & 0.893 & 95.8 & \textbf{69.6} & 89.2 \\
Flowgrad & 429 & 95.1 & 65.3 & 82.8 & 0.542 & 95.3 & 67.2 & 85.5 & 1.270 & 95.2 & 67.6 & 85.4 \\
EquiFM & 1438 & 98.6 & 87.4 & 94.8 & 1.593 & 98.6 & 87.4 & 94.8 & 6.873 & 98.6 & 87.3 & 94.8 \\ \bottomrule
\end{tabular}
}
\end{table}
